Distinguishing general relativity and $f(R)$ gravity with the gravitational lensing Minkowski functionals

We explore the Minkowski functionals of weak lensing convergence map to distinguish between $f(R)$ gravity and the general relativity (GR). The mock weak lensing convergence maps are constructed with a set of high-resolution simulations assuming different gravity models. It is shown that the lensing MFs of $f(R)$ gravity can be considerably different from that of GR because of the environmentally dependent enhancement of structure formation. We also investigate the effect of lensing noise on our results, and find that it is likely to distinguish F5, F6 and GR gravity models with a galaxy survey of $\sim3000$ degree$^2$ and with a background source number density of $n_g=30~{\rm arcmin}^{-2}$, comparable to an upcoming survey dark energy survey (DES). We also find that the $f(R)$ signal can be partially degenerate with the effect of changing cosmology, but combined use of other observations, such as the cosmic microwave background (CMB) data, can help break this degeneracy.

==> author.tex <==
\author{Ling Chenxiaoji} 
\author{Wang Qiao}
\author{Li Ran}
\affiliation{National Astronomical Observatories, Chinese Academy of Sciences, 20A Datun Road, Chaoyang, Beijing 100012, China}
\author{Li Baojiu}
\affiliation{Institute for computational Cosmology, Department of Physics, Durham University, South Road, Durham DH1 3LE, UK}
\author{Wang Jie}
\affiliation{National Astronomical Observatories, Chinese Academy of Sciences, 20A Datun Road, Chaoyang, Beijing 100012, China}
\author{Gao Liang}
\affiliation{National Astronomical Observatories, Chinese Academy of Sciences, 20A Datun Road, Chaoyang, Beijing 100012, China}
\affiliation{Institute for computational Cosmology, Department of Physics, Durham University, South Road, Durham DH1 3LE, UK}
%\affiliation[1]{Department of Computer Science, \LaTeX\ University}
%\affiliation[2]{Department of Mechanical Engineering, \LaTeX\ University}

